Ship trajectory planning method for reproducing human operation at ports

Among ship maneuvers, berthing/unberthing maneuvers are one of the most challenging and stressful phases for captains. Concerning burden reduction on ship operators and preventing accidents, several researches have been conducted on trajectory planning to automate berthing/unberthing. However, few studies have aimed at assisting captains in berthing/unberthing. The trajectory to be presented to the captain should be a maneuver that reproduces human captain's control characteristics. The previously proposed methods cannot explicitly reflect the motion and navigation, which human captains pay particular attention to reduce the mental burden in the trajectory planning. Herein, mild constraints to the trajectory planning method are introduced. The constraints impose certain states (position, bow heading angle, ship speed, and yaw angular velocity), to be taken approximately at any given time. The introduction of this new constraint allows imposing careful trajectory planning (e.g., in-situ turns at zero speed or a pause for safety before going astern), as if performed by a human during berthing/unberthing. The algorithm proposed herein was used to optimize the berthing/unberthing trajectories for a large car ferry. The results show that this method can generate the quantitatively equivalent trajectory recorded in the actual berthing/unberthing maneuver performed by a human captain.

==> for_Japanese_draft/title.tex <==

\twocolumn[
    % {\bf 日本船舶海洋工学会講演会論文集}
    \vspace{1em}
    \begin{center}
        {\fontsize{20pt}{0pt}
            % {\bf % タイトルフォントサイズ 18pt
            %     チェックポイントを有した経路を自動生成する\\
            %     離着桟経路計画アルゴリズム
            % }
            % {\bf % タイトルフォントサイズ 18pt
            %     チェックポイントを用いて \\
            %     離着桟経路を自動生成するアルゴリズム
            % }
            {\bf % タイトルフォントサイズ 18pt
                Ship trajectory planning method  \\
                for reproducing human operation at port
            }
        }
        \vspace*{5mm}\\
        {\fontsize{11pt}{12.5pt}{\selectfont % 著者フォントサイズ 10pt
            \begin{tabular}{lll}
                巣　山　　凜 & \qquad & 宮　内　新　喜  \\
                梅　田　直　哉 & \qquad & 牧　　敦　生  \\
            \end{tabular}
        }}
        \vspace{3mm} \\
        {\fontsize{10pt}{12.5pt}{\selectfont
            English title will be written here.
        }}
        \vspace{1mm} \\
        \textit{\textbf{Key Words}: Trajectory planning}
        \vspace{2mm}
    \end{center}
]

==> setting.tex <==

\smartqed  % flush right qed marks, e.g. at end of proof

% insert here the call for the packages your document requires
%\usepackage{latexsym}
% etc.
\usepackage[dvipdfmx]{color}
\usepackage{graphicx}
\usepackage[T1]{fontenc}
\usepackage{mathptmx}  % 本文(セリフ体)，数式の変数を Times 系に
\usepackage[scaled]{helvet}  % サンセリフ体を大きさ95%に調整した Helvetica 系に
\usepackage{courier}%  タイプライタ体を Courier New 系に
\usepackage[subrefformat=parens]{subcaption}
% \renewcommand{\thefigure}{\arabic{figure}}
% \renewcommand{\thetable}{\arabic{table}}

\makeatletter
\let\cl@chapter\undefined
\makeatletter
% \usepackage[numbers,sort&compress]{natbib}
\usepackage{amsmath,amssymb}   % for math commands
\usepackage{mathtools} % for math commands
\usepackage{cleveref}  % for clever reference
\Crefname{equation}{Eq.}{Eqs.}% 
\Crefname{figure}{Fig.}{Figs.}%
\usepackage{amsbsy}
\usepackage{bm}
\usepackage{algorithmic}
\usepackage{algorithm}
\providecommand{\argmin}{\operatornamewithlimits{argmin}} % argmin
\providecommand{\sensei}[1]{\textcolor{red}{Akimoto-sensei gosoudan point: #1}}


% show line numbers
\usepackage{lineno}
\newcommand*\patchAmsMathEnvironmentForLineno[1]{%
  \expandafter\let\csname old#1\expandafter\endcsname\csname #1\endcsname
  \expandafter\let\csname oldend#1\expandafter\endcsname\csname end#1\endcsname
  \renewenvironment{#1}%
     {\linenomath\csname old#1\endcsname}%
     {\csname oldend#1\endcsname\endlinenomath}}% 
\newcommand*\patchBothAmsMathEnvironmentsForLineno[1]{%
  \patchAmsMathEnvironmentForLineno{#1}%
  \patchAmsMathEnvironmentForLineno{#1*}}%
\AtBeginDocument{%
\patchBothAmsMathEnvironmentsForLineno{equation}%
\patchBothAmsMathEnvironmentsForLineno{align}%
\patchBothAmsMathEnvironmentsForLineno{flalign}%
\patchBothAmsMathEnvironmentsForLineno{alignat}%
\patchBothAmsMathEnvironmentsForLineno{gather}%
\patchBothAmsMathEnvironmentsForLineno{multline}%
}
\linenumbers

% show revision
\usepackage{ulem}
\newcommand{\Add}[1]{\textcolor{red}{#1}}
\newcommand\Erase{\bgroup\markoverwith{\textcolor{red}{\rule[.5ex]{2pt}{0.4pt}}}\ULon}
% \newcommand{\Add}[1]{\textcolor{black}{#1}}	%
% \newcommand{\Erase}[1]{\if0{#1}\fi}	%

% for table revision
\newcommand{\AddT}[1]{\color{red}{#1}}


% Insert the name of "your journal" with
\journalname{Journal of Marine Science and Technology}
%

==> setting_j.tex <==

% ページ設定
\pagestyle{empty}
\usepackage{geometry}
\geometry{
	top=20truemm,
	bottom=20truemm,
	left=20truemm,
	right=20truemm,
	ignoreheadfoot,
	columnsep=12truemm
}
\sloppy

% 本文のフォントは9pt，行送りは12.5pt
\setlength{\baselineskip}{12.5pt}  
\usepackage{titlesec}
% Section の見出しは10pt
\titleformat{\section}{\centering\large\sffamily}{\thesection.}{0.5em}{} 
\titlespacing{\section}{1em}{1em}{0em} %見出し前後の空白{左}{上}{本文との間}
% Subsection の見出し9pt
\titleformat{\subsection}{\sf}{\thesubsection}{0.5em}{} 
\titlespacing{\subsection}{1em}{0em}{0em} %見出し前後の空白{左}{上}{本文との間}
% Subsubsection の見出し9pt
\titleformat{\subsubsection}{\sffamily}{(\thesubsubsection)}{0.5em}{} 
\titlespacing{\subsubsection}{0em}{0em}{0em} %見出し前後の空白{左}{上}{本文との間}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{amsmath} % math formula
\usepackage{mathtools}
\usepackage{txfonts}
\usepackage{zxjatype} 
\usepackage{lmodern}
\usepackage{graphicx}
\usepackage{here} % show the figure on strict position
\usepackage{cite}
\usepackage{booktabs}
\usepackage{color} % colorize the character
\usepackage{caption}
\usepackage{subcaption}  % add caption to subfigure
\usepackage{hyperref} % URL hyperlink
\usepackage{newtxtext,newtxmath} % new times 
\renewcommand{\figurename}{Fig.} % change name of Figure
\renewcommand{\tablename}{Table}  % change name of Table
\usepackage{fontspec}
\setsansfont{Arial}
\newfontfamily{\cen}{QTSchoolCentury}
\usepackage{bm}
\usepackage{multirow}
\usepackage{textcomp}
\usepackage{todonotes}

\usepackage{algorithm}
% \usepackage{algorithmic}
% \usepackage{algorithmicx}
\usepackage{algpseudocode}

\usepackage{mathtools} % for math commands
\usepackage{cleveref}  % for clever reference
\Crefname{equation}{Eq.}{Eqs.}% 
\Crefname{figure}{Fig.}{Figs.}%
\Crefname{table}{Tab.}{Tabs.}
% \Crefname{algorithm}{Alg.}{Algs.}
\Crefformat{section}{#2#1#3節}


\captionsetup[figure]{format=plain, labelformat=simple, labelsep=quad, font=small} % caption style of figure
\captionsetup[table]{format=plain, labelformat=simple, labelsep=quad, font=small} % caption style of table

\newcommand{\argmax}{\mathop{\rm arg~max}\limits}
\newcommand{\argmin}{\mathop{\rm arg~min}\limits}

\newcommand{\markupdraft}[2]{% {#1: {color|display} command}{#2: desired color or text}
%  the next lines can be incommented, if respectively certain notes or coloring should disappear
    \ifthenelse{\equal{#1}{display}}{#2}{}%                 % display only in draft version
    \ifthenelse{\equal{#1}{color}}{\color{#2}}{}%           % colored only in draft (for \new command)
}
\newcommand{\TODO}[2][]{\markupdraft{display}{{\color{red}~\\\noindent== TODO: #2 {\color{yellow}(#1)} ==\\}}}

% subsubsubsection
\makeatletter
\newcommand{\subsubsubsection}{\@startsection{paragraph}{4}{\z@}%
  {1.0\Cvs \@plus.5\Cdp \@minus.2\Cdp}%
  {.1\Cvs \@plus.3\Cdp}%
  {\reset@font\sffamily\normalsize}
}
\makeatother
\setcounter{secnumdepth}{4}

\DeclareFontFamily{OT1}{pzc}{}
\DeclareFontShape{OT1}{pzc}{m}{it}{<-> s * [1.10] pzcmi7t}{}
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}

\makeatletter
\def\@cite#1#2{$^{\hbox{\scriptsize{#1\if@tempswa , #2\fi})}}$} % change cite's position

\def\thebibliography#1{%

\list
{\arabic{enumi})}{\settowidth\labelwidth{#1)}\leftmargin\labelwidth
 \advance\leftmargin\labelsep
 \usecounter{enumi}}
 \def\newblock{\hskip .11em plus .33em minus .07em}
 \sloppy
 \sfcode`\.=1000\relax}
\let\endthebibliography=\endlist

\makeatother

